Addressing Corpus Knowledge Poisoning Attacks on RAG Using Sparse Attention

Retrieval Augmented Generation (RAG) is a highly effective paradigm for keeping LLM-based responses up-to-date and reducing the likelihood of hallucinations. Yet, RAG was recently shown to be quite vulnerable to corpus knowledge poisoning: an attacker injects misleading documents to the corpus to steer an LLM's output to an undesired response. We argue that the standard causal attention mechanism in LLMs enables harmful cross-document interactions, specifically in cases of attacks. Accordingly, we introduce a novel defense approach for RAG: Sparse Document Attention RAG (SDAG). This is a block-sparse attention mechanism that disallows cross-attention between retrieved documents. SDAG requires a minimal inference-time change to the attention mask. We present an empirical evaluation of LLM-based question answering (QA) with a variety of attack strategies on RAG. We show that our SDAG method substantially outperforms the standard causal attention mechanism. We further demonstrate the clear merits of integrating SDAG with state-of-the-art RAG defense methods. Specifically, the integration results in performance that is statistically significantly better than the state-of-the-art.

==> tables/adversarial_dominant_cluster_analysis.tex <==


\begin{table}[t]
\centering

\scriptsize
\begin{tabular}{c | cc cc cc}
\toprule
\multirow{3}{*}{\textbf{Generator}} &
\multicolumn{2}{c}{\textbf{HotpotQA}} &
\multicolumn{2}{c}{\textbf{TriviaQA}} &
\multicolumn{2}{c}{\textbf{NQ}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 &
\SDAG{} & \CARG{} &
\SDAG{} & \CARG{} &
\SDAG{} & \CARG{} \\
\midrule

 Llama    &   \textbf{0.84} & 0.82& \textbf{0.90} &0.84  & \textbf{0.60}  & 0.55 \\

Qwen    &   \textbf{0.90} & \textbf{0.90} & \textbf{0.92} &0.91  &\textbf{0.68}     & \textbf{0.68}\\

 Mistral &  \textbf{0.90}&\textbf{0.90}& 0.91 &  \textbf{0.94}&   \textbf{0.67} & \textbf{0.67} \\



\bottomrule
\end{tabular}
\caption{
Dominant-set-based generation of AS for \SDAG{} and \CARG{}, using E5 and $\text{\K{}}=5$.
Boldface marks the best result for a generator and dataset; in all cases, \SDAG{} and \CARG{} are statistically significantly indistinguishable for a generator and dataset.
}
\label{tab:adversarial_dominant_cluster_analysis}
\end{table}


==> tables/dominant_cluster_by_datasets.tex <==
\begin{table}[t]
\centering

\setlength{\tabcolsep}{3.5pt}
\scriptsize
\begin{tabular}{c c | cc cc cc}
\toprule
\multirow{3}{*}{\textbf{\K{}}} &
\multirow{3}{*}{\textbf{Generator}} &
\multicolumn{2}{c}{\textbf{HotpotQA}} &
\multicolumn{2}{c}{\textbf{TriviaQA}} &
\multicolumn{2}{c}{\textbf{NQ}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & &
\SDAG{} & \CARG{} &
\SDAG{} & \CARG{} &
\SDAG{} & \CARG{} \\
\midrule

 \multirow{3}{*}{5}
 & Llama   
 & \textbf{0.67}$^*$ & 0.42
 & \textbf{0.77}$^*$ & 0.60
 & \textbf{0.70}$^*$ & 0.60 \\
 & Qwen    
 & \textbf{0.51} & 0.42
 & \textbf{0.69} & 0.66
 & \textbf{0.66} & 0.59 \\
 & Mistral 
 & \textbf{0.51}$^*$ & 0.40
 & \textbf{0.81}$^*$ & 0.70
 & \textbf{0.74}$^*$ & 0.64 \\

\cmidrule(lr){1-8}

 \multirow{3}{*}{10}
 & Llama   
 & \textbf{0.62}$^*$ & 0.38
 & \textbf{0.85}$^*$ & 0.66
 & \textbf{0.75}$^*$ & 0.63 \\
 & Qwen    
 & \textbf{0.60}$^*$ & 0.43
 & \textbf{0.76}$^*$ & 0.68
 & \textbf{0.73} & 0.69 \\
 & Mistral 
 & \textbf{0.75}$^*$ & 0.41
 & \textbf{0.91}$^*$ & 0.76
 & \textbf{0.92}$^*$ & 0.70 \\

\bottomrule
\end{tabular}
\caption{
Dominant-set-based generation of GTS for \SDAG{} and \CARG{}, using E5.
Boldface marks the best result for a \K{}, generator, dataset, and evaluation measure; ’$^*$’ marks a statistically significant difference between \SDAG{} and \CARG{} for a \K{}, generator, dataset, and evaluation measure.
}
\label{tab:dominant_cluster_across_datasets}
\end{table}

==> tables/instruction_following.tex <==


\begin{table}[t]
\centering
\caption{
Retrieved-Set-Answers (RSA) group proportion in RAG using \SDAG{} and \CARG{} in an \oracle{} setting, using Llama as generator.
Boldface marks the best result, and ’$^*$’ marks a statistically significant difference between methods for a retriever, \K{}, and dataset configuration using an unpaired t-test.
}
\label{tab:instruction_following}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\scriptsize
\begin{tabular}{c c | cc | cc | cc}
\toprule
\multirow{3}{*}{\textbf{Retriever}} & 
\multirow{3}{*}{\textbf{\K{}}} &
\multicolumn{2}{c|}{\textbf{NQ}} &
\multicolumn{2}{c|}{\textbf{TriviaQA}} &
\multicolumn{2}{c}{\textbf{HotpotQA}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & &
\SDAG{} & \CARG{} &
\SDAG{} & \CARG{} &
\SDAG{} & \CARG{} \\
\midrule

\multirow{2}{*}{E5}
 & {5}
 & \textbf{0.22}$^*$ & 0.13 & \textbf{0.72}$^*$ & 0.55 & \textbf{0.62} & 0.60 \\

 & {10}
 & \textbf{0.26}$^*$ & 0.11 & \textbf{0.71}$^*$ & 0.55 & 0.55 & 0.55 \\


\cmidrule(lr){1-8}

\multirow{2}{*}{Contriver}
 & {5}
 & \textbf{0.30} & 0.29 & \textbf{0.69} & 0.59 & 0.58 & \textbf{0.61} \\

 & {10}
 & \textbf{0.24} & 0.22 & \textbf{0.65}$^*$ & 0.53 & 0.49 & \textbf{0.60}$^*$ \\

 \cmidrule(lr){1-8}

\multirow{2}{*}{Okapi-BM25}
 & {5}
 & \textbf{0.46}$^*$ & 0.35 & \textbf{0.75}$^*$ & 0.53 & \textbf{0.74}$^*$ & 0.62 \\

 &{10}
 & \textbf{0.50}$^*$ & 0.31 & \textbf{0.74}$^*$ & 0.57 & \textbf{0.75}$^*$ & 0.62 \\

\bottomrule
\end{tabular}
\end{table}

